Loschmidt echo approach to Krylov-subspace approximation error estimation

The Krylov subspace method is a standard approach to approximate quantum evolution, allowing to treat systems with large Hilbert spaces. Although its application is general, and suitable for many-body systems, estimation of the committed error is involved. This makes it difficult to automate its use. In this paper, we solve this problem by realizing that such error can be regarded as a Loschmidt echo in a tight-binding Hamiltonian. We show that the different time-regimes of the approximation can be understood using simple physical ideas. More importantly, we obtain computationally cheap error bounds that describe with high precision the actual error in the approximation.

==> extras/anal_sol__version_juli_.tex <==
\section{ Analytical solution of the error: special case of homogeneous hopping} \label{sec:analytical}
Intro.

The particular case of homogeneous coefficients $\forall \alpha_i = \alpha$ and $\beta_i = \beta$ corresponds to the Toeplitz tridiagonal matrix \cite{toeplitz_matrix}. The model is easily written in the basis
\begin{equation}
    \label{eq:topelitz_hamiltonian}
    H_N=\sum_{n=1}^{N-1} \alpha \psi_{n} \psi_{n}^{*}+\beta\left(\psi_{n+1} \psi_{n}^{*}+\psi_{n} \psi_{n+1}^{*}\right)+\alpha \psi_{N} \psi_{N}^{*},
\end{equation}

The advantage in this situation comes from the well documented analytical solutions for the eigenvalues and eigenvectors, which are

\begin{equation}
    \label{eq:topelitz_eigenvectors}
\left\langle \psi_{n},\varphi_{k}\right\rangle =\sqrt{\frac{2}{N+1}}\sin\left(\frac{nk\pi}{N+1}\right),
\end{equation}

and 

\begin{equation}
        \label{eq:topelitz_eigenvalues}
\lambda_{k}=\alpha+2 \beta \cos \left(\frac{n k \pi}{N+1}\right).
\end{equation}


Let the echo of two time-evolutions with Toeplitz matrices of lengths $N$ and $N'$ be expressed as $LE_{N,N'} = \left\langle\psi_{0}\left|e^{-i t H_{N}^{\prime}} e^{i t H_{N}}\right| \psi_{0}\right\rangle$.
The time evolution of an initial state represented as $\psi(t=0)=\sum_{n=1}^N C_n \psi_n$

\begin{equation}
    \label{eq:topelitz_evolution}
    \begin{aligned}
        \psi(t) & =\sum_{n,n'}^{N}C_{n} S_{n,n'}^{N}(t)\psi_{n'}
    \end{aligned}
\end{equation},

where the transition matrix $S_{n,n^{\prime}}^N(t)$ it is define as 

\begin{equation}
    \label{eq:topelitz_transition_matrix}
    S_{n,n^{\prime}}^N(t) = \sqrt{\dfrac{2}{N+1}} \sum_{k=1}^{N}
    \sin\left(\frac{nk\pi}{N+1}\right)
    \sin\left(\frac{n'k\pi}{N+1}\right)
    e^{it\lambda_{k}}.
\end{equation}

Finally, replacing the evolved state into the Loschmdit echo expression yields

\begin{equation}
    \label{eq:topelitz_echo}
    1 - \left\langle\psi_{1}\left|
    e^{-i t H_{N}^{\prime}}
    e^{i t H_{N}}\right| \psi_{1}\right\rangle =
    \sum_{n=1}^{N^{\prime}} S_{1 n}^{N}(t) S_{n,1}^{N^{\prime}}(-t).
\end{equation}

Already from the eigenvalues (\ref{eq:topelitz_eigenvalues}), it is clear that the parameter $\alpha$ will not affect the value of the echo. On the other hand, $\beta$ acts as a rescaling of time. This way one can study the behavior of the chain with parameters $\alpha=0$ and $\beta=1$, and assign


% no me gusta realmente esta notacion pero va a quedar asi
% hasta que se nos ocurra una mejor

\begin{equation}
    \label{eq:topelitz_map_solutions}
    LE_{N,N^{\prime}}(t, \alpha,\beta) = 
    LE_{N,N^{\prime}}(\beta t, \alpha=0,\beta=1). 
\end{equation}

The fact that $\beta$ acts as a rescaling in time, it's heavily related to the range of validity for the Krylov approximation. And that this
determined by the dispersion of the Hamiltonian.

==> extras/beta.tex <==
\section{Estimation of the ocupation of site $N+1$}\label{sec:ap_beta}
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
This appendix is devoted to discuss the robustness of the approximation of the $\alpha_{N+1}$ and $\beta_{N+1}$ using Eq. \ref{app}. The amplitud of the evolved
state in the Lanczos basis is $\Braket{v_i|\psi_{D}} \equiv \psi_i$

%\Huge Idea para discutir:
%\normalsize
Estoy pensando como lo quiero decir
Basicamente queremos estimar la ocupacion del sitio N+1 en funcion de la
evolucion hasta ahora, y ver como cambia esta estimacion si cambia el $\beta$

Argumento 1: Nos interesa la zona exponecialmente decreciente a la derecha de la onda, esto nos da una relacion muy util 

\begin{equation}
    \psi_{k}(t) >> \psi_{k+1}(t) >> \psi_{k+2}(t)
\end{equation}

Esta relacion nos permite aproximar las ecuaciones de movimiento a orden cero en $\beta_k$ como.

\begin{align}
    \label{eq:ecuaciones_de_movimiento}
    i \frac{\partial}{\partial t}\psi_{1} &=
    \alpha_{1} \psi_{1} 
    + \beta_{1} \psi_{2}\\ \nonumber
    &\vdots\\ \nonumber
    i \frac{\partial}{\partial t}\psi_{k} &=
    \alpha_{k} \psi_{k}
    + \beta_{k-1} \psi_{k-1} 
    + \bcancel{\beta_{k} \psi_{k+1}} 
\end{align}

%Finalmente lo que nos da es una solucion para
%$\psi_{k}^{(0)}$ tal que
%$\psi_{k}^{(0)} = F[\psi_{k-1},\psi_{k-2},\psi_{k-3}, ...]$, lo importante de esta aproximacion es que $\psi_{k}$ no depende de $\psi_{k+1}$.

\begin{equation}
    i \frac{\partial}{\partial t}\psi_{k+1}^{(1)} =
    \alpha_{k+1} \psi_{k+1}^{(1)} 
    + \beta_{k} \psi_{k}^{(0)}
\end{equation}

%La solucion a esta ODE queda queda escrita en terminos de la %fuente ($\psi_{k}$) como una convolucion,

\begin{align}
    i \mathcal{L}[\psi_k^{\prime}] &= 
    \alpha_{k} \mathcal{L}[\psi_k] +
    \beta_{k} \mathcal{L}[\psi_{k+1}]\\ \nonumber
    \hat{\psi}_{k+1} &=
    i\beta_{k}
    \frac{\hat{\psi}_{k}}
    {s - i\alpha_{k} }\\
    \nonumber
   i\beta_{k} \mathcal{L}^{-1}
    \frac{\hat{\psi}_{k}}
    {s - i\alpha_{k} }\\
    \nonumber
    \psi_{k+1}^{(1)} &= i \beta_{k} 
    \left(
    \psi_{k}^{(0)}(t) * e^{it\alpha}
    \right)
\end{align}

Basicamente lo que nos dice eso es que a primer orden la ocupacion del ultimo estado es lineal en el beta.
Y la pendiente al hacer el cociente con el echo real es independiente del tiempo, asi que aproximarlo no es tan terrible. si vemos la figura de abajo, esto casi que se cumple. Pero la pendiente depende un poco del tiempo, parece una correccion a segundo orden 

Si queremos calular el error a orden dos en beta,
lo que tenemos que hacer es reemplazar la solucion encontrada para $\psi_{k+1}^{(1)}$ en \ref{eq:ecuaciones_de_movimiento}
Lo que nos quedaria

\begin{equation}
    i \frac{\partial}{\partial t}\psi_{k}^{(2)} =
    \alpha_{k} \psi_{k}^{(0)} 
    + \beta_{k-1} \psi_{k-1}^{(0)}
    + \beta_{k} \psi_{k+1}^{(1)}
\end{equation}

Si identificamos el primer termino como la derivada temporal de $\psi_{k}^{(0)}$, la solucion a esta ecuacion es simplemente.


\begin{equation}
    \psi_{k}^{(2)} = 
    \psi_{k}^{(0)}
    - \beta_{k}^2 
    \int_{0}^{t}
    \left(
    \psi_{k}^{(0)}(t^{\prime}) * e^{it^{\prime}\alpha}
    \right)
    d t^{\prime}
\end{equation}

Como la solucion con la cadena cortada es quedarse a orden cero en beta, es inmediato identificar el error a orden $2$ en $\beta_{k}$ como,

\begin{equation}
    e^{(2)}(t) = 
    i \beta_{k}
    \left(
    \psi_{k}^{(0)}(t) * e^{it\alpha}
    \right)
    - \beta_{k}^2 
    \int_{0}^{t}
    \left(
    \psi_{k}^{(0)}(t^{\prime}) * e^{it^{\prime}\alpha}
    \right)
    d t^{\prime}
\end{equation}

para hacer la notacion mas entendible,

\begin{equation}
    e^{(2)}(t) = 
     \beta_{k} g(t)
    +\beta_{k}^{2} f(t) 
\end{equation}

si queremos estudiar el error al aproximar $\beta_k$ por algun estiador $\hat{\beta_{k}}$ realtivo al error real lo que llegamos es que

\begin{equation}
    \frac{e^{(2)}_{\hat{\beta_k}}(t)}
    {e^{(2)}_{\beta_k)}(t)} =
    \frac{\hat{\beta_{k}}}
    {\beta_{k}}
    \left(
    \frac{1 + f(t)/g(t) \hat{\beta_{k}}}
    {1 + f(t)/g(t) \beta_{k}}
    \right)
\end{equation}

Ahora como $f(t)<<g(t)$, podemos esperar que esta relacion sea lineal con alguna correccion. 

Ahora hay que escribir esto de forma decente

\begin{figure}[H]
\includegraphics[scale=.25]{figures/BETAS.pdf}
\caption{Cociente entre el echo real y el aproximado para un beta, en funcion de ese beta sobre el beta real, para 4 tiempos distintos}
\label{fig:BETAS}
\end{figure}

%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%

==> extras/intro__old_.tex <==
\section{Introduction} \label{sec:introduction}
    
Transmitting and processing information in quantum devices has been established in recent years \cite{bruss2019quantum}. Laboratories around the world are in the race to develop increasingly accurate quantum devices.
To carry out this successfully, it is necessary to test their operation on classical devices.
For this reason, it is important to have efficient classical algorithms to perform quantum simulation \cite{PhysRevLett.88.097904, terhal2002classical}.
    
Several approaches for the efficient computation of quantum time-evolution have been proposed in the literature 
\cite{kluk1986comparison,SCHOLLWOCK201196,PhysRevA.78.012321,daley2004time,PhysRevLett.93.040502}. The cost of the simulation usually depends on specifics of the system, e.g. the initial state, or on the information that
we want to know about the dynamics.
For example, the cost of the simulation can be greatly reduced if the amount of entanglement 
developed by the system remains bounded \cite{daley2004time,PhysRevLett.93.040502}. 
Less restrictive are the well-known Krylov-subspace methods, constructed to provide approximations to the action of the exponential of a matrix on a vector. In the context of quantum simulation, the mechanics of the approximation is the following: an initial state in a (possibly very) large Hilbert space is first mapped to an effective subspace, the Krylov subspace, that captures the most relevant features of the dynamics. Within this low-dimensional subspace, time evolution is (cheaply) computed. Finally, the evolved state is mapped back to the large Hilbert space. Besides quantum simulation, the method has other important applications like solving systems
of ordinary differential equations, large-scale linear systems and more \cite{saad2003iterative,gazzola2020krylov}


The core challenge in Krylov-subspace methods is to keep the error limited, in order to achieve precise evolution. For this reason, it is desirable to be able to predict the time regime in which the error will remain less than a given predetermined tolerance. 
This problem
has been approached in several ways in the literature \cite{park1986unitary,saad1992analysis,stewart1996error,hochbruck1997krylov,expokit,moler2003nineteen,Jawecki:2020cc}, and the provided bounds
generally overestimate the error (significantly). In the seminal paper \cite{park1986unitary}, Park and Light use the fact that the dynamics
in the reduced subspace is that of an effective 1d lattice with a tridiagonal Hamiltonian. An initial state localized at one end starts spreading and the error in the approximation is approximated by the population in the other end of the chain. Later, Saad \cite{saad1992analysis} derived computable estimates of the error using an expansion in the Krylov subspace exploiting the
Lanczos algorithm. Other error bounds include involved computations
making it difficult to use in an operational way \cite{hochbruck1997krylov}.

The goal of this paper is to find tight and computationally inexpensive error bounds for the approximation error in Krylov schemes.
We take advantage of a simple observation: the error can be regarded as a Loschmidt echo in which both the forward and backward evolutions are given by tight-binding Hamiltonians. \martin{ In the forward case, the effective dimension is fixed by the Krylov-subspace while the 
backwards evolution occurs in a space of dimension of the Hilbert space of the system.}
This analogy allows us to describe the time-regimes of the error using well-known results in Loschmidt echo theory. In particular, we show that the error remains negligilbe up to some time, related with the effective traveling wave-packet  on the trimmed chain (of size given
by the size of the Krylov-subspace \cite{park1986unitary}) and its tail "colliding" with the last site. The core of our proposal is that the error in this regime can be ridiculously well captured by a backwards evolution in a chain with only one more site instead of the actual one with dimension of Hilbert space sites.
% The first one 
%can be related to the time it takes to cross a
%fictitious chain with nearest neighbor hopping of length given
%by the size of the Krylov-subspace \cite{park1986unitary}. Until that time the error is practically zero. Then,
%it grows abruptly. 
Moreover, we show that one can analytically solve the
error for the case in which the tight binding Hamiltonian has 
homogeneous diagonal and off-diagonal elements. It is shown that this solution works very well in a 1-D spin Ising spin chain with transverse magnetic field. Finally, we give some physical insight
explaining why this simple model works in the general case.

The paper is organized as follows. In Sec.\ref{sec:Krylov}, we introduce the Krylov-subspace method for quantum time evolution. Next, in Section. \ref{sec:regimes} we describe the different time-regimes of the error, focusing on the analogy with Loschmidt echo dynamics under tight-binding Hamiltonians.
In section \ref{sec:numres} we use the connection between the error and the Loschmidt echo of tight-binding Hamiltonians to propose an error bound that
describes extremely well the inaccuracy of the approximate evolution in the Krylov subspace.
Finally, Sec.\ref{sec:conclu} concludes with some final remarks. Appendix \ref{sec:ap_lanczos} provides a brief description of Lanczos algorithm to obtain an orthonormal basis spanning the Krylov subspace and in Appendix \Ref{sec:ap_ising} we describe the system that we use for the calculations, a 1-D Ising spin chain with transverse magnetic field. 
In Appendix \ref{sec:analytical}, the error is analytically solved for
the simplest case in which the tight-binding Hamiltonian has equal diagonal and non diagonal elements.


%One is a Krylov subspace obtained from a Lanczos iteration that maps the Heisenberg time-evolution generated by the Floquet Hamiltonian onto dy- namics of a single particle on a fictitious chain with nearest neighbor hopping. 


% Less restrictive are the well-known Krylov-subspace methods, which can be used to deal with the problem of approximating 
% the action of matrix exponential. 
% In this case, the key point is to approximately project the exponential operator from the large space of the system onto 
% a small effective subspace. Then, the exponential operation of the 
% evolution is performed in a much smaller matrix. This general method has other important applications as solving systems
% of ordinary differential equations, large-scale linear systems and more \cite{saad2003iterative,gazzola2020krylov}

==> extras/regime2.tex <==
\section{Numerical results} \label{sec:numres}


Sketch with the derivations so far of the expansion of the echo in the general case.\
First lets define what we want to calculate, in this case it's the Echo between a chain (tight binding) of length $N$ and the same chain but with one hopping parameterized with $\lambda$.
So we can write a general hamiltonian to work with as

\begin{equation}
    H_\lambda = (\sum_{n \neq k}^{N-1} \alpha_{n} P_{n,n} + 
    \beta_{n }P_{n,n+1})
    + \lambda P_{k,k+1} + \alpha_k P_{k,k} + \alpha_{N} P_{N,N}
\end{equation}

Where the projectors $P_{i,j}$ make the action of exchanging the state $\psi_{j}$ to $\psi_i$, and are defines as 

\begin{equation}
    P_{i,j} = \psi_{i} \psi_{j}^{\dagger} + \psi_{j} \psi_{i}^{\dagger}
\end{equation}

During this derivations the important object that appear are the commutators and anti commutators of this projectors. In doing so we find another set of anti hermitian operator $V_{i,j}$ witch are the antisymmetric analogous of the $P_{i,j}$.

\begin{align}
    \Big[ P_{a,b} , P_{c,d} \Big] = V_{a,d} \delta_{b,c} + 
                                    V_{a,c} \delta_{b,d} +
                                    V_{b,c} \delta_{a,d} +
                                    V_{b,d} \delta_{a,c}
\end{align}
